Arrangement Computation for Planar Algebraic Curves

We present a new certified and complete algorithm to compute arrangements of real planar algebraic curves. Our algorithm provides a geometric-topological analysis of the decomposition of the plane induced by a finite number of algebraic curves in terms of a cylindrical algebraic decomposition of the plane. Compared to previous approaches, we improve in two main aspects: Firstly, we significantly reduce the amount of exact operations, that is, our algorithms only uses resultant and gcd as purely symbolic operations. Secondly, we introduce a new hybrid method in the lifting step of our algorithm which combines the usage of a certified numerical complex root solver and information derived from the resultant computation. Additionally, we never consider any coordinate transformation and the output is also given with respect to the initial coordinate system. We implemented our algorithm as a prototypical package of the C++-library CGAL. Our implementation exploits graphics hardware to expedite the resultant and gcd computation. We also compared our implementation with the current reference implementation, that is, CGAL's curve analysis and arrangement for algebraic curves. For various series of challenging instances, our experiments show that the new implementation outperforms the existing one.

==> conclusion.tex <==
\eric{REWRITE SECTION}

future
\begin{itemize}
 \item various improvements conceivable
 \item gcds of resultants in bisolves
\end{itemize}


\eric{THIS IS ALENEX:}
We propose an exact and complete method to isolate the real solutions
of a bivariate polynomial system. Our algorithm is designed to
reduce the number of purely symbolic operations as much as possible.
Eventually, only resultant computation and square-free factorization of
the resultant polynomial are still needed. By transferring the
resultant computation to the GPU, we are able to remove a major
bottleneck of elimination approaches. In order to further improve our 
implementation, we aim to outsource the square-free factorization to the 
GPU as well, a step which seems to be feasible since factorization is also
well suited for a "divide-conquer-combine" modular approach.
Since our initial motivation was to speed up the topology and arrangement
computation for algebraic curves and surfaces, we plan to extend our method
towards this direction. Furthermore, it would be interesting to extend 
our algorithm to handle higher dimensional systems or complex solutions.
Finally, we would like to investigate in hybrid methods such as the 
combination of a numerical complex root solver and an exact post 
certification method serving as an additional filter in the validation step (in
the spirit of~\cite{strzebonski-cylindrical,r-tenmethods}). We are 
convinced that most of the candidate boxes could be treated even more 
efficiently by 
the use of such methods. We claim that, eventually, the  
total costs for solving a bivariate system should \emph{only} be dominated by 
those of the root isolation step for the elimination polynomial. For many 
instances, our experiments already hint to the latter claim. We aim to further 
improve our implementation to show this behavior for all instances and to 
provide a proof in terms of complexity as well.

